Simulation methods and error analysis for trawl processes and ambit fields

Trawl processes are continuous-time, stationary and infinitely divisible processes which can describe a wide range of possible serial correlation patterns in data. In this paper, we introduce new simulation algorithms for trawl processes with monotonic trawl functions and establish their error bounds and convergence properties. We extensively analyse the computational complexity and practical implementation of these algorithms and discuss which one to use depending on the type of L\'evy basis. We extend the above methodology to the simulation of kernel-weighted, volatility modulated trawl processes and develop a new simulation algorithm for ambit fields. Finally, we discuss how simulation schemes previously described in the literature can be combined with our methods for decreased computational cost.

==> old_algorithms/grid_discretisation.tex <==
\begin{algorithm}[h]
  \caption{grid discretization}%\label{algo:grid_discretisation}
    \begin{algorithmic}[1]
    \State Compute the $N \times N_s$ indicator matrix $I.$
      %\State generate the grid $\mathcal{G}_{\mathcal{R}_1}$ on $\mathcal{R}_1 = [\tau+T,\tau] \times [0,\phi(0)]$ and the indicator matrix $\{I_{ij}\}_{\substack{1 \le i \le N_t-1 \\ 1 \le j \le N_s-1}} $ with $I_{ij} = 1 $
      %if $g_{ij}$ is fully contained in $A_{\tau_1}$ and $0$ otherwise
      %  \State generate the grid $\mathcal{G}_{\mathcal{R}}$ on $\mathcal{R} = [s+T,ks] \times [0,\phi(0)]$ 
      \State Sample the $N \times N_s$ matrix $Y^1$ with iid entries $Y^1_{ij}$ which are equal in law to $L(c).$  
      \State Set $X_\tau = Y^1 \odot I. $
      \For{\text{each } $l\in\{2,\ldots,k\}$}
      \State Let $Y^l$ be given by the last $N-N_t$ columns of $Y^{l-1}$ together with $N_t$ new columns added to the right, where the new elements are also iid and equal in to law to $L(c).$
      \State Set $X_{l\tau} = Y^l \odot I.$
      \EndFor
  %\State sample the Gaussian and jump parts $\xi =\{\left(y_g,\tilde{y}_g\right)\}_{g \in \mathcal{G}_{\mathcal{R}}}$ according to \eqref{eq:simplified_cumulant}
 % \State convolve $\mathcal{G}_\mathcal{R}$ with $I$ with stride $N_t.$ 
  \end{algorithmic}
\end{algorithm}

==> pictures/slice/convolution.tex <==
\pgfkeys{tikz/mymatrixenv/.style={decoration={brace},every left delimiter/.style={xshift=8pt},every right delimiter/.style={xshift=-8pt}}}
\pgfkeys{tikz/mymatrix/.style={matrix of math nodes,nodes in empty cells,left delimiter={[},right delimiter={]},inner sep=1pt,outer sep=1.5pt,column sep=2pt,row sep=2pt,nodes={minimum width=20pt,minimum height=10pt,anchor=center,inner sep=0pt,outer sep=0pt}}}
\pgfkeys{tikz/mymatrixbrace/.style={decorate,thick}}

\newcommand*\mymatrixbraceright[4][m]{
    \draw[mymatrixbrace] (#1.west|-#1-#3-1.south west) -- node[left=2pt] {#4} (#1.west|-#1-#2-1.north west);
}
\newcommand*\mymatrixbraceleft[4][m]{
    \draw[mymatrixbrace] (#1.east|-#1-#2-1.north east) -- node[right=2pt] {#4} (#1.east|-#1-#2-1.south east);
}
\newcommand*\mymatrixbracetop[4][m]{
    \draw[mymatrixbrace] (#1.north-|#1-1-#2.north west) -- node[above=2pt] {#4} (#1.north-|#1-1-#3.north east);
}
\newcommand*\mymatrixbracebottom[4][m]{
    \draw[mymatrixbrace] (#1.south-|#1-1-#2.north east) -- node[below=2pt] {#4} (#1.south-|#1-1-#3.north west);
}

\begin{equation*}
\label{trawl_slice_eq}
    \tilde{Y} = 
    \begin{tikzpicture}[baseline={-0.5ex},mymatrixenv]
        \matrix [mymatrix,inner sep=5pt] (m)  
        {
        0  & \ldots  & 0 \\
        \vdots  & & \vdots   \\
        0 &   \ldots &  0 \\        
        L\left(S_{11}\right)  & \ldots &  L\left(S_{1k}\right) \\
        L\left(S_{21}\right)  &  \ldots &  L\left(S_{2k}\right)\\
         \vdots        &    & \vdots  \\
        L\left(S_{I1}\right) &  \ldots &  L\left(S_{Ik}\right)\\
};
        % Braces     
        \mymatrixbraceright{1}{3}{$I-1$}
        \mymatrixbraceright{4}{7}{$k$}
       % \mymatrixbracetop{1}{3}{$C'$}
        %\mymatrixbracetop{4}{6}{$C''$}
        %\mymatrixbracebottom{3}{3}{$F'$}
       % \mymatrixbracebottom{4}{4}{$F''$}
       % \mymatrixbraceleft{3}{3}{$E'$}
       % \mymatrixbraceleft{4}{4}{$E''$}
    \end{tikzpicture}
\end{equation*}


==> pictures/slice/convolution_non_compact.tex <==
\pgfkeys{tikz/mymatrixenv/.style={decoration={brace},every left delimiter/.style={xshift=8pt},every right delimiter/.style={xshift=-8pt}}}
\pgfkeys{tikz/mymatrix/.style={matrix of math nodes,nodes in empty cells,left delimiter={[},right delimiter={]},inner sep=1pt,outer sep=1.5pt,column sep=2pt,row sep=2pt,nodes={minimum width=20pt,minimum height=10pt,anchor=center,inner sep=0pt,outer sep=0pt}}}
\pgfkeys{tikz/mymatrixbrace/.style={decorate,thick}}

\renewcommand*\mymatrixbraceright[4][m]{
    \draw[mymatrixbrace] (#1.west|-#1-#3-1.south west) -- node[left=2pt] {#4} (#1.west|-#1-#2-1.north west);
}
%\newcommand*\mymatrixbraceleft[4][m]{
%    \draw[mymatrixbrace] (#1.east|-#1-#2-1.north east) -- node[right=2pt] {#4} (#1.east|-#1-#2-1.south east);
%}
%\newcommand*\mymatrixbracetop[4][m]{
%    \draw[mymatrixbrace] (#1.north-|#1-1-#2.north west) -- node[above=2pt] {#4} (#1.north-|#1-1-#3.north east);
%}
%\newcommand*\mymatrixbracebottom[4][m]{
%    \draw[mymatrixbrace] (#1.south-|#1-1-#2.north east) -- node[below=2pt] {#4} %}

\begin{equation*}
    \tilde{Y} = 
    \begin{tikzpicture}[baseline={-0.5ex},mymatrixenv]
        \matrix [mymatrix,inner sep=5pt] (m)  
        {
        0  & \ldots  & 0 & 0 \\
        \vdots  & & \vdots & \vdots  \\
        0 &   \ldots &  0 & 0 \\        
        L\left(S_{11}\right)  & \ldots & L\left(S_{1,k-1}\right) & L\left(S_{1k}\right) \\
        L\left(S_{21}\right)  &  \ldots &  L\left(S_{2,k-1}\right) & 0 \\
         \vdots &    \udots   &  \vdots  & \vdots  \\
        L\left(S_{k1}\right) &  \ldots &  0 & 0 \\
};
        % Braces     
        \mymatrixbraceright{1}{3}{$k-1$}
        \mymatrixbraceright{4}{7}{$k$}
       % \mymatrixbracetop{1}{3}{$C'$}
        %\mymatrixbracetop{4}{6}{$C''$}
        %\mymatrixbracebottom{3}{3}{$F'$}
       % \mymatrixbracebottom{4}{4}{$F''$}
       % \mymatrixbraceleft{3}{3}{$E'$}
       % \mymatrixbraceleft{4}{4}{$E''$}
    \end{tikzpicture}, \qquad   F = \begin{pmatrix}
    0 & 0 & \dots & 0 & 1 \\
    0 & 0 & \dots & 1 &1 \\
    \vdots & \vdots & \udots & \vdots & \vdots \\
    0 & 1 & \dots & 1 &1 \\
    1 & 1 & \dots & 1 & 1
  \end{pmatrix}. 
\end{equation*}


==> pictures/tikz_files/attempt_3.tex <==
\begin{tikzpicture}
\draw[->,ultra thick] (-6.5,0)--(0.5,0)  node[right]{$t$};
\draw[->,ultra thick] (0,0)--(0,7.5)     node[above]{$x$};
\node at (-1,0)
\draw[black,thick] (-5.65,0) node[anchor=north]{$T$}  -- (0,7) %node[anchor=north]{$C$}
-- (0,0) node[anchor=north]{$0$}
  -- cycle;
  
\draw[step=1cm,color=gray!75,opacity=0.5] (-6,0) grid (0,7);
%grid of cells contained in the trawl
\filldraw [fill=gray, draw=black,opacity=0.5] (-4,0)
-- (-4,2)
-- (-3,2)
-- (-3,3)
-- (-2,3)
-- (-2,4)
-- (-1,4)
-- (-1,5)
-- (0,5)
-- (0,0)
-- cycle;
\end{tikzpicture}


==> pictures/tikz_files/grid_approximation.tex <==
\begin{tikzpicture}
\draw[->,ultra thick] (-6.5,0)--(3.5,0)  node[right]{$t$};
\draw[->,ultra thick] (0,0)--(0,7.5)     node[above]{$x$};
\draw[black,thick] (-6.0,0) node[anchor=north]{$l\tau + T$}  -- (0,7) %node[anchor=north]{$C$}
-- (0,0) node[anchor=north]{$l\tau$}
  -- cycle;

\node at (-5.35,1.3) {$g^l_{21}$};
\node at (-5.35,0.3) {$g^l_{11}$};
\node at (-4.35,0.3) {$g^l_{12}$};
\node at (-3.35,0.3) {$g^l_{13}$};
  
\draw[step=1cm,color=gray!75,opacity=0.5] (-6,0) grid (0,7);
%grid of cells contained in the trawl
\filldraw [fill=gray, draw=black,opacity=0.5] (-5,0)
-- (-5,1)
-- (-4,1)
-- (-4,2)
-- (-3,2)
-- (-3,3)
-- (-2,3)
-- (-2,4)
-- (-1,4)
-- (-1,5)
-- (0,5)
-- (0,0)
-- cycle;
\end{tikzpicture}

==> pictures/tikz_files/grid_theorem_3.tex <==
%check the other overlefa document for the version that renders correctly
\begin{tikzpicture}
\begin{axis}[axis lines=right,  
    axis x line=middle,
    xlabel={$t$},
    ylabel={$x$},
    %position spatial axes label on top of the axis
    every axis y label/.style={
       at={(ticklabel* cs:1.05)},
       anchor=south,
    },
    xtick={-7, ..., -1},
    ytick={0,0.2,...,1.1},
    domain=-7:0,
    xmin=-7, xmax=0,
    ymin=0, ymax=1.1,
    samples=50,
    scale only axis,
    width=7cm, height=5.5cm
]
\addplot+[mark=none,color=black] {e^(x/2.75)};

\draw[step=1cm,color=gray!75,opacity=0.5] (-3,0) grid (0,1);
\filldraw [fill=gray, draw=black,opacity=0.5]
-- (-3,0)
-- (-3,0.2)
-- (-2,0.2)
-- (-2,0.4)
-- (-1,0.4)
-- (-1,0.6)
-- (0,0.6)
-- (0,0)
-- cycle;
\end{axis}
\end{tikzpicture}

==> pictures/tikz_files/grid_update_tikz.tex <==
\begin{tikzpicture}
\draw[->,ultra thick] (0,0)--(10,0) node[right]{$t$};
\draw[->,ultra thick] (0,0)--(0,7.5) node[above]{$x$};
%1st trawl
\draw (1.5,0) node[anchor=north]{$l\tau+T$}
  -- (6.5,7) %node[anchor=north]{$C$}
  -- (6.5,0) node[anchor=north]{$l\tau$}
  -- cycle;
%2nd trawl
\draw (4,0) node[anchor=north]{$(l+1)\tau+T$}
  -- (9,7) %node[anchor=north]{$C$}
  -- (9,0) node[anchor=north]{$(l+1)\tau$}
  -- cycle;
%remove grid
\filldraw [fill=gray, draw=black,opacity=0.5] (4,0)
-- (1.5,0)
-- (1.5,7)
-- (4,7)
-- (4,0)
-- cycle;
\node at (2.75,4) {\shortstack{{\LARGE remove}\\$G_l \backslash G_{l+1}$}};
%keep grid
\filldraw [fill=gray, draw=black,opacity=0.2] (4,0)
-- (4,0)
-- (4,7)
-- (6.5,7)
-- (6.5,0)
-- cycle;
\node at (5.25,4) {\shortstack{{\LARGE keep}\\$G_l \cap G_{l+1}$}};
%add grid
\filldraw [fill=gray, draw=black,opacity=0.5] (4,0)
-- (6.5,0)
-- (6.5,7)
-- (9,7)
-- (9,0)
-- cycle;
\node at (7.75,4) {\shortstack{{\LARGE add}\\$G_{l+1} \backslash G_l$}};
\end{tikzpicture}
